Interpretations of SUSY Searches in ATLAS with Simplified Models

We present the status of interpretations of Supersymmetry (SUSY) searches in ATLAS at the Large Hadron Collider (LHC) using simplified models. Such models allow a systematic scan through the phase space in the sparticle mass plane, and in the corresponding final state kinematics. Models at various levels of simplification have been studied in ATLAS. The results can be extrapolated to more general new physics models which lead to the same event topology with similar mass hierarchies. Searches in the no-lepton channel with 1.04 fb^-1 of data from 2011 and the same-sign dilepton channel with 35 pb^-1 of data from 2010 are presented. No excess above the Standard Model expectation is observed, and the results are interpreted using the simplified models.

==> nolep.tex.v2 <==
\section{No-lepton Search}

The SUSY search with all-hadronic and \met ~signature
(so called ``No-lepton Mode'') is considered to be one of 
the ``golden channels.'' It has the largest coverage over
possible phase space of R-parity conserving pMSSM 
models~\cite{rizzo}.

In this search, three simplified models are considered as shown 
in Figure~\ref{fig:simplifiedModel_nolep}, where 
gluinos and light-flavor squarks are initially pair-produced. 
Direct decays to the lightest supersymmetric particles (LSPs)
are considered, which are the simplest decays contributing to 
the no-lepton channel~\cite{alwall}. 

\if0
\begin{figure}[t]
\centering
\includegraphics[width=120mm]{figures/simplifiedModel_nolep.eps}
\caption{Simplified models considered for the no-lepton channel.} 
\label{fig:simplifiedModel_nolep}
\end{figure}
\fi

\begin{figure} [t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.3\linewidth]{figures/simplifiedNoLep_4j.eps}
\includegraphics[width=0.3\linewidth]{figures/simplifiedNoLep_3j.eps} 
\includegraphics[width=0.3\linewidth]{figures/simplifiedNoLep_2j.eps}
\end{tabular}
\caption{Simplified models considered for the no-lepton channel, where 
gluinos and squarks directly decay down to the LSP in the gluino-gluino (left),
gluino-squark (center), and squark-squark (right) processes.}
\label{fig:simplifiedModel_nolep}
\end{figure}

Five signal regions are considered to cover various regions of the
gluino-squark mass plane as shown in Table~\ref{tab:0lep_SR}.
First of all, events are discarded if electrons and muons with $\pt > 20$ GeV
remain. In order to suppress detector noise and non-collision 
background, events are required to have the primary vertex 
associated with at least five tracks, and are discarded if 
any jets fail quality selection criteria described in ~\cite{jetcleaning}.
Cuts on \met ~and the leading jet $p_T$ are applied to be on the efficiency 
plateau of the trigger requirement. Further selections on the sub-leading
jets are considered to cover event topologies from $\tilde{q}\tilde{q}$, 
$\tilde{g}\tilde{q}$, and $\tilde{g}\tilde{g}$ processes, where
the final states consist of at least two, three, and four jets respectively.  
Effective mass ($\meff$) is defined as the scalar sum of \met and the $\pt$
of the two, three, four leading, or all the jets with $\pt>40$~GeV used for 
each signal region.
It is known to be approximately proportional to the mass of initially produced 
sparticles~\cite{Meff}. 
$\Delta \phi(\textrm{jet},\ptmiss)_\mathrm{min}$ and $\met/\meff$ cuts are 
applied to suppress the QCD background. Two signal regions are considered
for the four-jet case using different requirements on $\meff$ to cover 
smaller and larger mass splittings between the sparticles. 


\begin{table}[t]
  %\small
  \begin{center}\renewcommand\arraystretch{1.2}
\renewcommand\tabcolsep{1.2mm}
    \begin{tabular}{| l l | c|c|c|c|}
 \hline \hline
 & Signal Region &$\geq$ 2-jet & $\geq$ 3-jet & $\geq$ 4-jet & High mass \\
% & Signal Region & A & B & C  \\ %rev
\hline
\hline
& $\met$            & $>130$ &  $>130$ &  $>130$  & $>130$ \\ 
& Leading jet $\pt$       & $>130$ &  $>130$ &  $>130$  & $>130$ \\ 
\hline
& Second jet      $\pt$   & $>40$ &  $>40$ &  $>40$ & $>80$\\ 
& Third jet      $\pt$       &  --         &  $>40$ &  $>40$ & $>80$\\ 
& Fourth jet      $\pt$       &  --        &     --       &  $>40$ & $>80$\\ 
\hline
&$ \Delta \phi(\textrm{jet},\ptmiss)_\mathrm{min}$ & $>0.4$ & $>0.4$  & $>0.4$ & $>0.4$   \\ 
& $\met / \meff$     & $>0.3$     & $>0.25$ & $> 0.25$ & $>0.2$ \\ 
& $\meff$   & $>1000$  &  $>1000$ & $>500/1000$ & $>1100$ \\ 
\hline \hline
\end{tabular}
\caption{Event selection for each of the five overlapping signal regions ($\meff$, energy and momentum in GeV).
 Note that $\meff$ is defined with a variable number of jets, appropriate to each signal region. In the high mass selection, all jets with $\pt>40$~GeV are used to compute the $\meff$ value used in the final cut. The $\Delta \phi(\textrm{jet},\ptmiss)_\mathrm{min}$ cut is only applied up to the third leading jet. }
    \label{tab:0lep_SR}
  \end{center}
\end{table}


Dominant sources of background from Standard Model processes are  
W+jets, Z+jets, top pair, multi-jet and single top production. 
Non-collision background is found to be negligible. 
%explanations for BG

In order to estimate the backgrounds fully or partially in data-driven 
ways, five control regions (CRs) are defined for each of the five
signal regions (SRs), which are designed to provide uncorrelated data 
samples enriched with particular background sources. 
The observations in the CRs are used to estimate the background 
expectations in the SRs by using transfer factors, 
which are the ratios of expected event counts in the CR and SR
derived independently from the CR and SR themselves. 
The transfer factors are obtained from MC simulations 
for the W+jets, Z+jets, top backgrounds, whereas for the multijet
background, it is fully derived from data by smearing jets in 
the low \met ~events with jet response functions as is done
in~\cite{daCosta}.

For the Z+jets background, irreducible
contributions from Z($\rightarrow \nu \bar{\nu}$)+jets are dominant. 
Two CRs are considered that are enriched with $\gamma+$jets and 
Z($\rightarrow e^+ e^-, \mu^+ \mu^-$)+jets, 
%using data from the single photon or lepton trigger, 
which have similar 
kinematics. The momentum of the photon or the dilepton system from 
Z is added to the $\ptmiss$ to reproduce the \met ~distribution of the
Z($\rightarrow \nu \bar{\nu}$)+jets process. 

The W($\rightarrow l \nu$)+jets and top backgrounds are 
estimated from events containing one lepton 
and with \met $>$ 130 GeV. Furthermore, the 
transverse mass $M_T = \sqrt{2 p_T^l p_T^{\nu} (1 - \cos \Delta \phi(l,\nu))}$ 
is computed by assuming that the measured \met ~provides the neutrino information, and
is required to 
be between 30 GeV and 100 GeV to select W and top events. 
The events are then separated into two CRs 
using the b-tagging information, where jets arising from b-quarks
are identified using the impact parameter and secondary
vertex information. 
The lepton in the events is treated as a jet when computing 
the kinematic variables, since the dominant sources of W+jets 
and top backgrounds contain W's decaying into hadronic taus and 
tau-neutrinos.

Finally, for the multijet background, the control region is 
chosen such that the cut on $\Delta \phi(\textrm{jet},\ptmiss)_\mathrm{min}$
is reversed and tightened to 
$\Delta \phi(\textrm{jet},\ptmiss)_\mathrm{min} < 0.2$.
In such events, $\ptmiss$ is aligned with jets in the 
transverse plane, and \met ~originates from the mismeasurement of jets
or neutrino emission from heavy flavor decays within jets. 
An additional and separate CR was considered to estimate the 
impact of the dead region in the LAr EM barrel calorimeter. 

For the transfer factors derived from the MC simulation, important sources of 
systematic uncertainties are the jet energy scale, jet energy 
resolution, MC modeling uncertainties such as renormalization and 
factorization scale and parton distribution function (PDF) uncertainties, 
and uncertainty arising from the presence of pile-up. 
Additional uncertainties originate from photon and lepton trigger and
reconstruction efficiencies, photon and lepton energy scale and 
resolution (for estimating the W+jets, Z+jets, and top backgrounds),  
b-tag/veto efficiency (for W+jets and top), photon acceptance 
and background (for Z+jets), and MC statistics. For the data-driven
estimation of the multijet background, the main source of uncertainties
for the transfer factor is the modeling of the non-Gaussian tail
of the jet response function. 

%\begin{figure}[t]
%\centering
%\includegraphics[width=80mm]{figures/0lep_evsel.eps}
%\caption{Five signal regions for the no-lepton search.} 
%\label{fig:0lep_evsel}
%\end{figure}

\begin{table*}[t]
\small
\begin{center}
%\renewcommand\arraystretch{1.4}
\begin{tabular}{|c|c|c|c|c|c|}
\hline\hline
\multirow{2}{*}{Process}     &\multicolumn{5}{|c|}{Signal Region} \\ 
\cline{2-6} & \multirow{2}{*}{$\ge 2$-jet} & \multirow{2}{*}{$\ge 3$-jet} & $\ge 4$-jet,  & $\ge 4$-jet,  & \multirow{2}{*}{High mass} \\ 
                                           & & & $\meff>500$~GeV & $\meff>1000$~GeV & \\ \hline \hline
$Z / \gamma$+jets & $ 32.5\pm 2.6\pm 6.8$ & $ 25.8\pm 2.6\pm 4.9$ & $ 208\pm 9\pm 37$ & $ 16.2\pm 2.1\pm 3.6$ & $  3.3\pm 1.0\pm 1.3$ \\
 $W$+jets &$ 26.2\pm 3.9\pm 6.7$ &$ 22.7\pm 3.5\pm 5.8$ &$ 367\pm30\pm126$ &$ 12.7\pm 2.1\pm 4.7$ &$  2.2\pm 0.9\pm 1.2$ \\
$t\bar{t}$+ Single Top  &$  3.4\pm 1.5\pm 1.6$ &$  5.9\pm 2.0\pm 2.2$ &$ 375\pm37\pm 74$ &$  3.7\pm 1.2\pm 2.0$ &$  5.6\pm 1.7\pm 2.1$ \\
QCD jets   &$ 0.22\pm0.06\pm0.24$ &$ 0.92\pm0.12\pm0.46$ &$  34\pm 2\pm 29$ &$ 0.74\pm0.14\pm0.51$ &$ 2.10\pm0.37\pm0.83$ \\ \hline

Total  &$ 62.3\pm 4.3\pm 9.2$ &$  55 \pm 3.8\pm 7.3$ &$ 984\pm39\pm145$ &$ 33.4\pm 2.9\pm 6.3$ &$ 13.2\pm 1.9\pm 2.6$ \\ \hline \hline

Data  & 58 & 59 & 1118 & 40 & 18 \\

  \hline\hline
 \end{tabular}
\caption{\label{tab:SRevc} Fitted background components in each SR, compared with the observation. 
In each case the first (second) quoted uncertainty is statistical (systematic). Estimates of background 
components are partially correlated and hence the uncertainties (statistical and systematic) on the total 
background estimates do not equal the quadrature sums of the uncertainties on the components. }
 \end{center}
 \end{table*}


Table~\ref{tab:SRevc} shows the numbers of Standard Model background
events expected in the signal regions, and the numbers of observed
events. The \meff ~distributions are shown in Figure~\ref{fig:0lep_meff} for 
each signal region. No excess is observed, and thus limits are obtained 
for each channel. The $\text{CL}_\text{s}$ prescription is used to set the 
exclusions. 
Figure~\ref{fig:0lep_limits} 
shows the combined exclusion limits 
for the simplified models with $m_{\text{LSP}} = 0$. 

%\begin{figure}[t]
%\centering
%\includegraphics[width=80mm]{figures/0lep_bkg.eps}
%\caption{Estimates of background components for the no-lepton search.} 
%\label{fig:0lep_bkg}
%\end{figure}
%\input{table2.tex}


\begin{figure} [p]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.4\linewidth]{figures/0lep_Meff_2j.eps}
\includegraphics[width=0.4\linewidth]{figures/0lep_Meff_3j.eps} \\
\includegraphics[width=0.4\linewidth]{figures/0lep_Meff_4j.eps}
\includegraphics[width=0.4\linewidth]{figures/0lep_Meff_4jHM.eps} 
\end{tabular}
\caption{The \meff ~distributions for the dijet (top left), three jet (top
right), four jet (bottom left), and four jet high mass (bottom right) 
channels.}
\label{fig:0lep_meff}
\end{figure}

\begin{figure}[p]
\centering
\includegraphics[width=80mm]{figures/0lep_combined_limits.eps}
\caption{Combined exclusion limit for the simplified models with 
$m_{\text{LSP}} = 0$. The red bold line shows the observed limit at 95\%
CL, and the blue dashed line corresponds to the median expected 95\% CL 
limit. The dotted blue lines show the expected 68\% and 99\% CL expected
limits. } 
\label{fig:0lep_limits}
\end{figure}



==> table2.tex <==
\begin{table*}[t]
\small
\begin{center}
%\renewcommand\arraystretch{1.4}
\begin{tabular}{|c|c|c|c|c|c|}
\hline\hline
\multirow{2}{*}{Process}     &\multicolumn{5}{|c|}{Signal Region} \\ 
\cline{2-6} & \multirow{2}{*}{$\ge 2$-jet} & \multirow{2}{*}{$\ge 3$-jet} & $\ge 4$-jet,  & $\ge 4$-jet,  & \multirow{2}{*}{High mass} \\ 
                                           & & & $\meff>500$~GeV & $\meff>1000$~GeV & \\ \hline \hline
$Z / \gamma$+jets & $ 32.3\pm 2.6\pm 6.9$ & $ 25.5\pm 2.6\pm 4.9$ & $ 209\pm 9\pm 38$ & $ 16.2\pm 2.2\pm 3.7$ & $  3.3\pm 1.0\pm 1.3$ \\
 $W$+jets &$ 26.4\pm 4.0\pm 6.7$ &$ 22.6\pm 3.5\pm 5.6$ &$ 349\pm30\pm122$ &$ 13.0\pm 2.2\pm 4.7$ &$  2.1\pm 0.8\pm 1.1$ \\
$t\bar{t}$+ single top  &$  3.4\pm 1.6\pm 1.6$ &$  5.9\pm 2.0\pm 2.2$ &$ 425\pm39\pm 84$ &$  4.0\pm 1.3\pm 2.0$ &$  5.7\pm 1.8\pm 1.9$ \\
QCD multi-jet   &$ 0.22\pm0.06\pm0.24$ &$ 0.92\pm0.12\pm0.46$ &$  34\pm 2\pm 29$ &$ 0.73\pm0.14\pm0.50$ &$ 2.10\pm0.37\pm0.82$ \\ \hline

Total  &$ 62.4\pm 4.4\pm 9.3$ &$  54.9\pm 3.9\pm 7.1$ &$ 1015\pm41\pm144$ &$ 33.9\pm 2.9\pm 6.2$ &$ 13.1\pm 1.9\pm 2.5$ \\ \hline \hline

Data  & 58 & 59 & 1118 & 40 & 18 \\

  \hline\hline
 \end{tabular}
\caption{\label{tab:SRevc} Fitted background components in each SR, compared with observation. The $Z/\gamma$+jets background is constrained by CR1a and CR1b, the QCD multi-jet, $W$ and top quark backgrounds by CR2, CR3 and CR4, respectively. In each case the first (second) quoted uncertainty is statistical (systematic). Estimates of background components are partially correlated and hence the uncertainties (statistical and systematic) on the total background estimates do not equal the quadrature sums of the uncertainties on the components. }
 \end{center}
 \end{table*}


==> table3.tex <==
\begin{table*}
\small
\begin{center}\renewcommand\arraystretch{1.4}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline\hline
\multirow{2}{*}{}     &\multicolumn{6}{|c|}{ Signal / Control Region} \\ 
\cline{2-7}
& CR1a & CR1b & CR2 & CR3 & CR4 & SR \\ 
\hline
\hline
Data  &8 &7 &34 & 15&12 & 18 \\ \hline
Targeted background  & $Z/\gamma$+jets& $Z/\gamma$+jets &  QCD multi-jet & $W$+jets &$t\bar{t}$ + single top &-- \\ \hline
Transfer factor &0.374 &0.812 &0.063 & 0.196&0.372 &--  \\ \hline
Fitted $Z/\gamma$+jets  &8.3 &5.8 &0.7 & 0.5&0.0& 3.3 \\
Fitted QCD multi-jet    &-- &-- &29.8 &0.8&0.6 & 2.1 \\ 
Fitted $W$+jets &-- &-- &0.5 & 10.0&0.4 & 2.1 \\
Fitted $t\bar{t}$ + single top  &-- &0.0 &3.0 & 3.7&11.0 & 5.7 \\ \hline
Fitted total background  &8.3 &5.9  &34.0  &15.0&12.0   & 13.1 \\
Statistical uncertainty   & $\pm$2.7 &$\pm$1.2 &$\pm$5.8 &$\pm$3.9 &$\pm$3.5 &$\pm$1.9 \\
Systematic uncertainty  & $\pm$0.6 &$\pm$1.7 &$\pm$0.1 &$\pm$0.1 &$\pm$0.2 & $\pm$2.5 \\
  \hline\hline
 \end{tabular}
\caption{\label{tab:SREdetails} Numerical inputs to and outputs from the likelihood fit to the control regions for the high mass channel. The transfer factor listed in the third row applies to the main targeted background for the CR, listed in the second row. An entry `--' in rows 5--7 indicates that the process in that row is assumed not to contribute to the control region (based on Monte Carlo studies) and hence is excluded from the fit. All numerical entries refer to event counts, with the exception of the transfer factors in the fourth row.}
 \end{center}
 \end{table*}

